Scaling Local Self-Attention for Parameter Efficient Visual Backbones

Self-attention has the promise of improving computer vision systems due to parameter-independent scaling of receptive fields and content-dependent interactions, in contrast to parameter-dependent scaling and content-independent interactions of convolutions. Self-attention models have recently been shown to have encouraging improvements on accuracy-parameter trade-offs compared to baseline convolutional models such as ResNet-50. In this work, we aim to develop self-attention models that can outperform not just the canonical baseline models, but even the high-performing convolutional models. We propose two extensions to self-attention that, in conjunction with a more efficient implementation of self-attention, improve the speed, memory usage, and accuracy of these models. We leverage these improvements to develop a new self-attention model family, HaloNets, which reach state-of-the-art accuracies on the parameter-limited setting of the ImageNet classification benchmark. In preliminary transfer learning experiments, we find that HaloNet models outperform much larger models and have better inference performance. On harder tasks such as object detection and instance segmentation, our simple local self-attention and convolutional hybrids show improvements over very strong baselines. These results mark another step in demonstrating the efficacy of self-attention models on settings traditionally dominated by convolutional models.

==> broader_impact.tex <==
\section*{Broader Impact}

% Much of the evolution of image models has started with ImageNet~\cite{russakovsky2015imagenet}, and percolated into other, and perhaps more practical, vision tasks such as detection, instance segmentation, keypoint estimation.
% Our hope is that these results will translate well into practical applications of vision models.
% In an ideal world, we would like to see applications of our work in addressing important vision problems on large images.

Our work is focused on studying how self-attention can be used to improve image classifiers.
The history of computer vision has repeatedly shown that improvements in image classification readily percolate to other computer vision tasks.
Thus, we take the view that our work will directly impact many vision tasks.
These improvements may benefit several important problems, such as automated medical image diagnosis, better prediction of weather from satellite imagery, and autonomous driving.
However, these models can also exhibit failure modes, such as misclassifications or predictions that reinforce biases inherent in the training data, among other fairness issues.
Furthermore, these technologies may used to automate tasks with far reaching societal consequences, such as surveillance.
On the whole, we believe that improving computer vision models, along with fair data curation and ethical frameworks that tackle the use of these technologies, will help address many societal problems.

%such as medical diagnosis, weather prediction, etc.

==> deleted_stuff.tex <==
% \textbf{\begin{tabular}[c]{@{}c@{}}Spatial Extent\\ ($k \times k$)\end{tabular}}
\iffalse
\begin{table}[]
\centering
\begin{tabular}{cccc}
    \toprule
    \textbf{Query Block Size} & \textbf{Halo Size} & \textbf{Window Size} & \textbf{Accuracy (\%)} \\
    \midrule
    \multirow{4}{*}{$4\times4$}      & $1\times1$                & $6\times6$                  & 79.0                   \\
                              & $2\times2$                & $8\times8$                  & 79.6                   \\
                              & $3\times3$                & $10\times10$                & 79.8                   \\
                              & $4\times4$                & $12\times12$                & 80.2                   \\
    \midrule
    \multirow{4}{*}{$8\times8$}      & $1\times1$                & $10\times10$                & 79.7                   \\
                              & $2\times2$                & $12\times12$                & 80.2                   \\
                              & $3\times3$                & $14\times14$                & 80.5                   \\
                              & $4\times4$                & $16\times16$                & 80.5                   \\
    \bottomrule
\end{tabular}
\caption{
    \textbf{Increasing window size improves performance, while query block size does not affect performance.}
    Accuracy as a function of the window parameters of the attention layer. 
    As the window size increases, performance consistently increases (top to bottom for each query block size).
    Furthermore, a fixed window size performs consistently regardless of the query block size (see last two rows of $4\times4$ and first two rows of $8\times8$).
    }
\label{table:experiments:query-vs-halo}
\end{table}
\fi


\iffalse
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{query_vs_halo_diagram.pdf}
    \caption{
        \textbf{Larger halos uses more memory, while larger query blocks are asymmetric.}
        These diagrams depict a window size of 5 on a 1D input, but the same arguments apply for 2D images.
        Dark borders indicate the boundaries of a query block.
        Gray blocks are padding.
        \textbf{(a)} A query block size of 1 and halo size of 2 uses more memory than a query block size of 3 and halo size of 1.
        In general, for the same window size, larger halos use more memory and computation.
        \textbf{(b)} The sole query in a query block size of 1 sees a symmetric region around it, while non-centered queries in a query block size larger than 1 see an asymmetric region around it.
        In general, the larger the query block size, the larger the asymmetric skew.
    }
    \label{fig:experiments:query-vs-halo}
\end{figure}
\fi


\iffalse
\begin{table}[]
\centering
\begin{tabular}{l|cc|c}
\toprule
\textbf{Model}   & \textbf{Top-1} & \textbf{Top-5 } & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}\#Params\\ (Millions)\end{tabular}}} \\
  & \multicolumn{2}{c|}{\textbf{(\%)}}                 &                                                                                         \\
\midrule
HaloNet-A0 & 77.6 & 93.7 & 5.5 \\
EfficientNet-B0 & 77.3 & 93.5 & 5.3 \\
\hline
HaloNet-A1 & 79.9 & 94.9 & 8.1\\
EfficientNet-B1 & 79.2 & 94.5 & 7.8 \\
\hline
HaloNet-A2   & 80.4  & 95.1  & 9.4  \\
EfficientNet-B2  & 80.3  & 90.5   & 9.2  \\
Inception-v4   & 80.0  & 90.5 & 48.0  \\
\hline
HaloNet-A3   & 82.0  & 95.9  & 12.3  \\
EfficientNet-B3  & 81.7  & 95.6  & 12.0   \\
ResNeXt-101 & 80.9   & 95.6    & 84.0   \\
\hline
HaloNet-A4  & 83.1   & 96.5  & 19.1  \\
EfficienetNet-B4 & 83.0  & 96.3   & 19.0   \\
SENet   & 82.7  & 96.2   & 146.0 \\
AmoebaNet-A  & 82.7   & 96.1   & 87.0  \\
PNASNet   & 82.9   & 96.2   & 86.0 \\
\hline
HaloNet-A5   & 83.8   & 96.5  & 30.7  \\
EfficientNet-B5  & 83.7  & 96.7  & 30.0 \\
AmoebaNet-C  & 83.5 & 96.5     & 155.0 \\
\hline
HaloNet-A6  & 84.1  &  96.8  & 43.4 \\
EfficientNet-B6  & 84.2  &  96.8 &   43  \\
\bottomrule              
\end{tabular}
\caption{\textbf{HaloNet models perform competitively with the leading models.}}
\end{table}

\fi


\begin{table}[]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}HaloNet \\ Model \end{tabular}}} & \textbf{\BlockSize} & \textbf{\HaloSize} & \textbf{\VFactor} & \textbf{\BottleneckFactor} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Total \\ Layers \end{tabular}}} & \textbf{\ThirdGroupLayers} & \textbf{\ImageSize} & \textbf{\FinalFCWidth} &\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Params \\ (M)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}EfficientNet \\ Params (M)\end{tabular}}} \\
 & & & & & & & & & & \\
\midrule
A0     & 8 &  3 & 1.0 & 0.5 & 50 & 7 &224 & -- & 5.5 & 5.3\\
A1     & 8 & 3  & 1.0 & 1.0 & 59 & 10 & 256 & -- & 8.1 & 7.8 \\
A2     & 8 & 3  & 1.0 & 1.25 & 62 & 11 & 256 & -- & 9.4 & 9.2 \\
A3     & 10 & 3 & 1.0  & 1.5 & 65 & 12 & 320 & 1024 & 12.3 & 12 \\
A4     & 12 & 3 & 1.0  & 3 & 65  & 12 & 384 & 1280 & 19.1 & 19\\
A5     & 14 & 2 & 2.5  & 2 & 98  & 23 & 448 & 1536 & 30.7 & 30\\
A6     & 16 & 2 & 3 & 2.75 & 101 & 24 & 512 & 1536 & 43.4 & 43\\
\bottomrule
\end{tabular}
\caption{\textbf{We grow our models to match the parameters of the corresponding EfficientNet models}}
    \label{tab:experiments:model-description}
\end{table}


\iffalse
\begin{figure}
    \centering
    % \begin{minipage}[b]{0.49\textwidth}
        \includegraphics[width=0.75\textwidth]{images/image_scaling.pdf}
    % \end{minipage}%
    \caption{\textbf{With virtually no increase in parameters, HaloNet scales better for larger images using larger receptive fields} We annotate the graph with the block, halo sizes for each of the image settings. }
    \label{fig:image-scaling}
\end{figure}
\fi

\begin{abstract}
\iffalse
  Self-Attention has proved to be the dominant computational primitive in natural language processing. Its ability to model long-range dependencies with content based interactions has led to significant improvements in both language generation and understanding. In recent years, supervised computer vision has also seen benefits from using self-attention to model long-range interactions in tasks such as instance segmentation, object detection, and image classification. Recent papers have shown that self-attention models have better accuracy vs computation and accuracy vs parameter tradeoffs than convolutional models. While promising, self-attention models for classification still lag significantly behind the state-of-the-art models (SoTA) such as EfficientNet. We present \emph{HaloNet}, a self-attention model for image classification that achieves 84.2\% top-1 accuracy on the Imagenet benchmark, which is competitive with the best models on this task. We also present algorithms that improve the efficiency of local 2D self-attention for computer vision. On Tensor Processing Units (TPUs), a leading accelerator for deep learning workloads, our best HaloNet models are significantly faster than EfficientNet B7, without much drop in the accuracy. Our work is the first to show that self-attention models for image classification can be competitive with SoTA approaches.
  \fi
% Recent papers have shown initial promise of using self-attention based models for supervised vision where they use a local 2D blocks, similar to convolutions, which are parameter efficient. However, they lag significantly behind current state-of-the-art approaches ...
% In this work, we remove the existing limitations of self-attention by proposing a new layer that can scale to much larger receptive fields with both speed and memory improvements while still being parameter efficient. We propose a novel model called the HaloNet, which achieves ... on ImagetNet. We also systematically studying scaling properties of HaloNet with respect to receptive field and image sizes and achieve 84.2\% Top-1 Accuracy 




% 


% (1): Hook
% In recent years, supervised computer vision has also seen benefits from using self-attention to model long-range interactions in tasks such as instance segmentation, object detection, and classification.
% (1) Attention as a core primitive for computer vision has shown <something> promise 

% (2): Why should a vision practitioner care about attention:
%  Two properties:
% Parameter-independent scaling of receptive field
%  => allows larger receptive fields without increasing model size
%  => large images are used in detection, segmentation, and other classification tasks like medical imaging.
% Content-based interactions
%  => convolution is translation equivariant
%  => may improve expressiveness because it's like a content based parameterization locally connected network

% (3): Historical Context
% Recent papers have shown that pure self-attention models have better accuracy vs computation and accuracy vs parameter tradeoffs than convolutional models. 
% Recent papers have demonstrated that pure self-attention models improve the  accuracy vs computation and accuracy vs parameter tradeoffs over medium-sized baseline convolutional models. 

% (4): Problem
% 
% Existing works demosntrate promising gains on simple models  
%
% While recent papers on pure self-attention models have shown promising improvements in accuracy-computation and accuracy-parameter tradeoffs, it remains to be demonstrated that pure self-attention models can scale and match state-of-the-art convolutional networks.  
% Achieving scale with pure self-attention can be challenging due to large step times and memory usage if not carefully implemented.
% Guided by the need for efficiency and scaling
% While promising, self-attention models for classification still lag significantly behind the state-of-the-art models (SoTA) such as EfficientNet. 
% The current versions also can't scale receptive fields effectively and self-attention is much slower in speed compared to CNNs
%

% (5) This paper
% 
% In this work, we show that pure self-attention models can be competitive with the best convolutional models for classification.
%
% The diff: 
% 1 modeling change (striding), notion of blocks and halo
% Efficient algorithm for haloing allowing us to scale
% understanding regularizations for self-attention (for example SE not working)

% (6) How we do it
% To achieve this, we use a combination of (a) simple modeling changes, (b) an efficient algorithm for local 2D self-attention, (c) understanding the effect of modern regularizations on self-attention networks.

% Taking an / Inspired by / Build off existing self-attention model

% To bridge this gap 

% (6) Additionally
% scaling attention models wrt iamge size , receptive field
% nice scaling properties of parameters
% big model regime advantages (speed + parameters)
%In this work, we scale up pure self-attention models by proposing a novel algorithmic implementation that doubles the speed of large models and improves the memory consumption by xx\% .


% Methods

% The implementation of convolution has improved significantly over the course of past decade (see Section \ref{sec:related-works} for details).
% In contrast, attention is earlier in the implementation trajectory, and does not \emph{currently} have the same optimizations available.
% For example, implementations of convolution automatically handle window gathering logic, taking care to pipeline memory accesses and computation among other optimizations.
% However, generic implementations of window gathering are unavailable in modern deep learning libraries, requiring under-optimized manual implementations.

% Due to under-optimized implementation, self-attention vision models can be nontrivially slower and memory intensive than convolutional models, slowing down research and making it challenging to deploy in production environments.
% Thus, an important direction is to improve the implementation of self-attention vision models.
% In this section, we describe modifications to the implementation of local 2D attention in order to improve speed and memory usage.
% We focus on improving the performance on TPUs \citep{jouppi2017datacenter}, and leave it to future work to improve performance on other hardware platforms such as CPUs and GPUs.

% The window gathering operation, manually implemented for local 2D attention, can be a source of slowness and large memory usage.
% \citet{ramachandran2019standalone} used a series of data formatting operations to gather windows, but data formatting operations is expensive on TPUs.
% \todo{Is it known that sasa paper uses data formatting to implement local 2d? or we point to a previous implementation in t2t or not mention it?}
% The data formatting operations, such as transposes, reshapes, slices, and concatenations, take 40\% of the running time of the self-attention model in \citet{ramachandran2019standalone}.
% The model can be sped up by removing data formatting operations, as described in Figure \ref{fig:experiments:blocking-implementation}.

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}[b]{0.49\linewidth}
%         \includegraphics[width=1.0\textwidth]{sasa_blocking.pdf}
%         \caption{}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.49\linewidth}
%         \includegraphics[width=1.0\textwidth]{halonet_blocking.pdf}
%         \caption{}
%         \vspace{0.26cm}
%     \end{subfigure}
%     \caption{
%         \textbf{Data formatting operations can be removed by keeping the activation in a blocked representation, and by using convolutions to gather local context.}
%         \textbf{(a)} depicts the implementation of \citet{ramachandran2019standalone}, where the local 2D attention implementation performs blocking at the beginning and un-blocking at the end in order to avoid changing the implementation of other operations (e.g., BatchNorm).
%         The context gathering implementation uses explicit padding, slices, and concatenations which impose nontrivial costs on TPUs.
%         \textbf{(b)} In contrast, our implementation keeps the input and output in a blocked format, saving multiple reshapes and transposes.
%         We change the implementation of other operations to accomodate the blocked representation.
%         Furthermore, since convolutions are extremely well optimized on TPUs compared to data formatting operations, they can be used to gather the appropriate context by leveraging using a binary kernel with a single $1$ per output channel.
%         Other optimizations (not pictured) include using optimized einsums to implicitly perform reshapes and transposes alongside computation (e.g., when mixing attention heads), and implementing striding within attention itself as opposed to a post-attention average pool used in \citet{ramachandran2019standalone}.
%     }
%     \label{fig:experiments:blocking-implementation}
% \end{figure}

% By implementing these optimizations, the speed and memory usage of the operation is improved, as seen in Figure \ref{fig:methods:running-time-improvements}.
% Per step running time is improved by up to 45\% and memory usage is reduced by up to 75\%.
% These improvements make self-attention models more practical, and enable training larger models that was previously prohibitively expensive.
% We note that additional optimizations, such as fused operations and better pipelining of memory accesses with computation, can significantly improve the performance characteristics of the model, and we leave these to future work.

% ==

% In convolution, the windowing is done by the low level operation itself. 
% They are typically implemented in a way that minimizes additional memory usage and repeated computation.
% However, a general windowing primitive does not exist, and it must be done as part of the model implementation itself. 
% The process of manually creating windows relies on the data formatting operations of transposes, reshapes, slices and concatenations, which can be expensive for compute-optimized devices \todo{"compute optimized" is weird}.
% We want to minimize these transpose and reshape operations.

% Describe the typical way of doing it \citep{ramachandran2019standalone}:
% * get 4D input [batch, height, width, channels]
% * reshape and transpose into query blocks
% * slice and concat the halo region from neighboring query blocks to form memory blocks
% * compute Q from query block and K, V from memory block
% * do attention to get output with the same shape as query block
% * reshape back into 4D input to pass into other operations. 

% Each conversion between 4D and 5D input requires two reshapes and 1 transpose:
% * input = [batch, height, width, channels]
% * reshape into [batch, num-height-blocks, block-height, num-width-blocks, block-width, channels] where num-height-blocks = height / block-height and num-width-blocks = width / block-width
% * transpose into [batch, num-height-blocks, num-width-blocks, block-height, block-width, channels]
% * reshape into [batch, num-height-blocks, num-width-blocks, block-height * block-width, channels]
% %* reshape into [batch * num-height-blocks * num-width-blocks, block-height * block-width, channels]
% Attention is done within each [..., block-height * block-width, channels] block.
% This is 4D to 5D, 5D to 4D requires undoing these operations, but still has same number of data formatting costs.

% %\todo{do we have to do that last reshape? It seems like you could do QK = einsum('nhwijd, nhwabd -> nhwijab') followed by tf.nn.softmax(QK, axis=[-1, -2]) followed by out = einsum('nhwijab, nhwabd -> nhwijd'). I don't know what happens internally though -- perhaps a reshape is done internally? Maybe it would be good to look at how the TF / pytorch op is actually implemented}

% \todo{do we talk about heads?}

% The reshapes to 4D after the end of the attention op is done to maintain compatibility with other standard operations that expect 4D input, such as batch normalization, activation functions, and 1x1 convolutions.
% However, the key insight is that by modifying the non-attention operations to work with a 5D input, we don't have to convert between 4D and 5D operations, avoiding the data transfers.
% This simple change improves speed by up to XX\% and reduces memory consumption by up to YY\%, as seen in Figure zz.

% We need to combat the halo-ing problem because slices and concatenations can be slow.
% Since the data access pattern is regular, we can take advantage of fast implementations of convolution to gather the neighborhood.
% The data gathering can be implemented as a 3D convolution with a kernel that has 0s and 1s.
% The idea is demonstrated in 1D in Figure xx, and the idea straightforwardly extends to the 5D input.
% This change additionally improves speed by XX\% and reduces memory consumption by up to YY\%, as seen in Figure zz.

% \todo{this part is weird because we do reshape / transposes for the 3D conv, which is fused by XLA -- do we have to talk about that? Or can we be hazy and mention that we just do a convolution with a binary matrix.}
% \todo{do we mention padding?}

% Figure zz: two bar charts, one for speed and one for memory consumption. Has TPU and GPU numbers. Y axis is percentage improvement, where SASA is at 1.0. X axis is GPU / TPU. Per chart, there are three bars: (1) SASA, (2) 5D trick (but still using slice / concat), (3) Full halo. 
% \todo{Could also consider doing this with convolutions at different points.}

% For a particular query, the region it has access to is asymmetric. 
% Previously, in order to maintain spatial invariance, a mask was applied during the softmax computation to zero out the weights for keys that are outside a square neighborhood.
% This is a waste of computation, so in this work, we embrace asymmetric regions.
% This introduces a design choice of how asymmetric a model should be.
% For the same total region size, a small query block and large halo is more symmetric but more memory.
% There is definitely some formula of average asymmetry -- figure it out.
% In the experiments section, we experiment with the tradeoff in ablations.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1.0\textwidth]{running_time_improvements.pdf}
%     \caption{\textbf{Removing data formatting costs can greatly speed up running time on accelerators.} \todo{Figure is generated from fake numbers} Benchmarking a 3-4-6-3 model with image size = 256. Adding 5D data format improves models by xx\%. Using convolutions for data gathers further improves performance by yy\%. }
%     \label{fig:methods:running-time-improvements}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \begin{minipage}[b]{0.49\textwidth}
%         \centering
%         \includegraphics[width=1.0\textwidth]{running_time_improvements.pdf}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}[b]{0.49\textwidth}
%         \centering
%         \includegraphics[width=1.0\textwidth]{batch_size_improvements.pdf}
%     \end{minipage}
%     \caption{\textbf{Removing data formatting costs can greatly speed up running time and memory usage on accelerators.} \todo{Figure is generated from fake numbers} Benchmarking a 3-4-6-3 model with image size = 256. Adding 5D data format improves models by xx\%. Using convolutions for data gathers further improves performance by yy\%. }
%     \label{fig:methods:running-time-improvements}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\textwidth]{block_attention.pdf}
%     \caption{
%         \textbf{Attention is performed on a query block with surrounding context taken from neighboring query blocks.}
%         For efficiency, the input is initially grouped into \emph{query blocks}, where the query block size is $2\times2$ in the figure.
%         The \emph{context} for a query block is the query block itself alongside neighboring pixels from bordering query blocks.
%         In the attention computation, the queries $Q$ are generated from the query block while the keys $K$ and values $V$ are generated by the context, all through 3 different linear projections.
%         The output is computed with the standard attention equations on $Q$, $K$, $V$.
%         In practice, relative attention is also used in the attention computation (not depicted in the figure).
%         \prajit{Move K slightly to the left. Add subscripts to d ($d_{qk}$ and $d_v$). Increase darkness of the shape information. Relative attention?}
%     }
%     \label{fig:methods:attention}
% \end{figure}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\textwidth]{receptive_field.pdf}
%     \caption{
%         \textbf{}
%     }
%     \label{fig:methods:receptive-field}
% \end{figure}
% \begin{verbatim}
%   \usepackage[pdftex]{graphicx} ...
%   \includegraphics[width=0.8\linewidth]{myfile.pdf}
%\end{verbatim}

% \begin{itemize}
%     \item We should talk about strided attention
%     \item we shoudl talk about what HaloNet-50 is
%     \item should establish notation about $d_q, d_k, d_v$.
%     \item should establish notation about base width
%     \item establish notation about all hyperparameters that will be used in the ablation in table 1
%     \item fixed dims per head and why that decision was made
%     \item for the deeper models, we went for 3, 3, ... instead of 3, 4, for speed. Explain that. 
% \end{itemize}


\iffalse
\begin{itemize}
    \item \architecturemodule{\textbf{Squeeze-and-Excitation}} \citep{hu2018squeeze}: a channel attention module used after the spatial convolution. Originally benchmarked across a wide variety of convolutional models, including ResNets and Inception networks.
    \item \architecturemodule{\textbf{Swish}} \citep{ramachandran2017searching}: an activation function, $x \cdot \text{sigmoid}(\beta x)$.
    We set $\beta = 1$ following EfficientNet.
    Originally discovered by automated search techniques that used a ResNet.
    \item \regularization{\textbf{RandAugment}} \citep{cubuk2019randaugment}: a data augmentation scheme that simplifies AutoAugment \citep{cubuk2019autoaugment}, which was used in EfficientNet. Originally benchmarked on ResNets and EfficientNets.
    \item \regularization{\textbf{Label Smoothing}} \citep{szegedy2016rethinking}: trains networks with a soft label computed by mixing a one-hot distribution of the true label with a uniform distribution over all classes. Orignally benchmarked on the Inception architecture.
\end{itemize}
\fi


% \begin{table}[]
%     \small
%     \begin{tabular}{l|cc|cc}
%     \toprule
%     \multicolumn{1}{l|}{\textbf{Components}} & \textbf{\begin{tabular}[c]{@{}c@{}}HaloNet \\ Accuracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Baseline\\ $\Delta$\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}ResNet \\ Accuracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Baseline\\ $\Delta$\end{tabular}} \\
%     \midrule
%     Baseline  & 78.6 & 0.0 & 77.6 & 0.0   \\
%     \midrule
%     + LS & 79.8 & 1.2   & 78.1 & 0.5 \\
%     + LS, RA  & 80.3  & 1.7  & 77.8 & 0.2 \\
%     + SE  & 78.7  & 0.1  & 78.6  & 1.0 \\
%     + SE, Sw  & 78.8 & 0.2& 78.9 & 1.3 \\
%     + LS, SE  & 79.6 & 1.0 & 78.9 & 1.3\\
%     + LS, SE, Sw & 79.8 & 1.2 & 79.1 & 1.5  \\
%     + LS, SE, Sw, RA & 80.5  & 1.9& 79.3  & 1.7\\       
%     \bottomrule
%     \end{tabular}
%     \caption{
%       \textbf{HaloNet improves more than ResNet with regularizations, but does not improve significantly with architectural modules that strongly benefit ResNet.} 
%       Starting from a baseline model, adding \regularization{label smoothing (\textbf{LS})}, \regularization{RandAugment (\textbf{RA})}, \architecturemodule{Squeeze-and-Excitation (\textbf{SE})}, and \architecturemodule{Swish (\textbf{Sw})}.
%       A standard ResNet-50 is used for ResNet, and the HaloNet swaps all spatial convolutions in the ResNet with attention.
%       Regularizations improve HaloNet more than ResNet (e.g., see "+ LS, RA"), while architectural modules improve ResNet more than HaloNet (e.g., see "+ SE, Sw").
%     }
%     \label{table:experiments:component-ablation}
% \end{table}

% \begin{table}[]
% \small
% \begin{tabular}{l|cc|cc}
% \toprule
% \textbf{.} & \multicolumn{2}{c|}{\textbf{Values}} & \textbf{Accuracy} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Baseline \\ $\Delta$\end{tabular}}} \\& \textbf{Baseline}  & \textbf{Scaled}       &  &  \\
% \midrule
% %Baseline & 1.0 & 1.0  & 80.5 & 0.0 \\
% $\ThirdGroupLayers$ & 50 & 98 & 81.4 & 0.9 \\
% $\VFactor$  & 1.0 & 3.0 & 81.0 & 0.4 \\
% $\BaseWidthFactor$& 1.0  & 1.25 & 80.9 & 0.3 \\
% $\BottleneckFactor$ & 4.0  & 6.5 & 80.6 & 0.1 \\
% $\QKFactor$  & 1.0 & 6.5 & 80.3 & -0.2 \\
% \bottomrule
% \end{tabular}
%     \caption{\textbf{Increasing the number of channels for the values and number of layers has the most impact on accuracy.}}
%     \label{table:experiments:scaling}
% \end{table}
%Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
%Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
%who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
%biases in the data. If authors believe this is not applicable to them, authors can simply state this.

%Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}

% \newfloatcommand{capbtabbox}{table}[][\FBwidth]

% \begin{figure}
% \begin{floatrow}
% \ffigbox{%
%     \includegraphics[width=0.47\textwidth]{step_time_and_peak_memory_vertical.pdf}%
% %   \rule{3cm}{3cm}%
% }{%
%   \caption{\textbf{Optimizations improve performance.} Computed with Cloud TPU v3.}%
% }
% \capbtabbox{%
% \small
% \begin{tabular}{cc}
%     \toprule
%      \textbf{\begin{tabular}[c]{@{}c@{}}Output\\Resolution\end{tabular}}  & \textbf{Layers}                                                                                                                                                                             \\
%     \midrule
%     \LayerImageSize{4} & \begin{tabular}[c]{@{}c@{}}$7 \times 7$ conv stride 2, 64\\ $3 \times 3$ max pool stride 2\end{tabular}                                                                                   \\
%     \midrule
%     \LayerImageSize{4} & \LayerStructure{64}{3} \\
%     \midrule
%     \LayerImageSize{8} & \LayerStructure{128}{3} \\
%     \midrule
%     \LayerImageSize{16} & \LayerStructure{256}{\ThirdGroupLayers} \\
%     \midrule
%     \LayerImageSize{32} & \LayerStructure{512}{3} \\
%     \midrule
%     \LayerImageSize{32} & $1\times1, \FinalFCWidth$ \\
%     \midrule
%     $1\times1$  & \begin{tabular}[c]{@{}c@{}} global average pooling \\ fc, 1000 \end{tabular} \\
%     \bottomrule
% \end{tabular}
% }{%
%   \caption{\textbf{HaloNet model family specification.}}%
% }
% \end{floatrow}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1.0\textwidth]{step_time_and_peak_memory.pdf}
%     \caption{
%         \textbf{Optimizations improve step time and memory usage across all models.}
%         Benchmarking the results of optimizing the implementation of local self-attention.
%         All numbers of measured on a Cloud TPU v3 with a total batch size of 256.
%         The red line denotes the unoptimized model, and lower numbers are better.
%         Train step times improve significantly across all models, with a 55\% improvement for the smallest model.
%         Furthermore, peak memory usage is decreased by up to 22\%, enabling larger batch sizes.
%     }
%     \label{fig:experiments:speed-memory-improvements}
% \end{figure}


% \begin{table}[]
% \centering
% \begin{tabular}{cc}
%     \toprule
%     \textbf{Output Resolution}                & \textbf{Layers}                                                                                                                                                                             \\
%     \midrule
%     \LayerImageSize{4} & \begin{tabular}[c]{@{}c@{}}$7 \times 7$ conv stride 2, 64\\ $3 \times 3$ max pool stride 2\end{tabular}                                                                                   \\
%     \midrule
%     \LayerImageSize{4} & \LayerStructure{64}{3} \\
%     \midrule
%     \LayerImageSize{8} & \LayerStructure{128}{3} \\
%     \midrule
%     \LayerImageSize{16} & \LayerStructure{256}{\ThirdGroupLayers} \\
%     \midrule
%     \LayerImageSize{32} & \LayerStructure{512}{3} \\
%     \midrule
%     \LayerImageSize{32} & $1\times1, \FinalFCWidth$ \\
%     \midrule
%     $1\times1$  & \begin{tabular}[c]{@{}c@{}} global average pooling \\ fc, 1000 \end{tabular} \\
%     \bottomrule
% \end{tabular}
% \caption{
%     \textbf{HaloNet structure mimics ResNets.}
%     Notation: image size $\ImageSize$, attention query block size $\BlockSize$, attention halo size $\HaloSize$, attention output width multiplier $\VFactor$, bottleneck output width multiplier $\BottleneckFactor$, number of bottleneck blocks in group three $\ThirdGroupLayers$, final $1 \times 1$ conv width $\FinalFCWidth$.
% }
% \label{table:methods:network-structure}
% \end{table}
